Real-time Monte Carlo Denoising with Weight Sharing Kernel Prediction Network

Real-time Monte Carlo denoising aims at removing severe noise under low samples per pixel (spp) in a strict time budget. Recently, kernel-prediction methods use a neural network to predict each pixel's filtering kernel and have shown a great potential to remove Monte Carlo noise. However, the heavy computation overhead blocks these methods from real-time applications. This paper expands the kernel-prediction method and proposes a novel approach to denoise very low spp (e.g., 1-spp) Monte Carlo path traced images at real-time frame rates. Instead of using the neural network to directly predict the kernel map, i.e., the complete weights of each per-pixel filtering kernel, we predict an encoding of the kernel map, followed by a high-efficiency decoder with unfolding operations for a high-quality reconstruction of the filtering kernels. The kernel map encoding yields a compact single-channel representation of the kernel map, which can significantly reduce the kernel-prediction network's throughput. In addition, we adopt a scalable kernel fusion module to improve denoising quality. The proposed approach preserves kernel prediction methods' denoising quality while roughly halving its denoising time for 1-spp noisy inputs. In addition, compared with the recent neural bilateral grid-based real-time denoiser, our approach benefits from the high parallelism of kernel-based reconstruction and produces better denoising results at equal time.

==> RepVGG.tex <==
\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=1.0\linewidth]{Figures/RepVGG.pdf}
  %
  \caption{\label{fig:RepVGG}
           Different layer compositions of \textit{RepVGG Block}. It has a multi-branches structure at the training-time (left) and a single-branch structure at the inference-time (right).
           }
\end{figure}

==> RepVGG_block.tex <==
\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=1.0\linewidth]{Figures/RepVGG_block.pdf}
  %
  \caption{\label{fig:RepVGG_block}
           Different layer compositions of RepVGG Block. In training-time, the inputs are identically sent to 3 branches and the outputs are fused with an element-wise addition before the ReLU layer (left). In inference-time, the branches are replaced with one single equivalent convolutional layer (right).
           }
\end{figure}

==> RepVGG_parameter.tex <==
\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=1.0\linewidth]{Figures/RepVGG_parameter.pdf}
  
  %
  \caption{\label{fig:RepVGG_parameter}
           Structural re-parameterization between training-time and inference-time \ren{training and inference phase should be labeled in the Fig.}. We use single-channel input and output case for illustration, where the parameters of the $5 \times 5$ kernel size Conv layer can be represented as a $5 \times 5$ matrix (up), and it is similar for $3 \times 3$ and $1 \times 1$ Conv layers after padding with zero values (presented with empty grid cell). In inference-time, we construct one single $5 \times 5$ convolutional parameters with an element-wise addition(down).
           }
\end{figure}
